Bringing Clustering to MLL: Weakly-Supervised Clustering for Partial Multi-Label Learning

Label noise in multi-label learning (MLL) poses significant challenges for model training, particularly in partial multi-label learning (PML) where candidate labels contain both relevant and irrelevant labels. While clustering offers a natural approach to exploit data structure for noise identification, traditional clustering methods cannot be directly applied to multi-label scenarios due to a fundamental incompatibility: clustering produces membership values that sum to one per instance, whereas multi-label assignments require binary values that can sum to any number. We propose a novel weakly-supervised clustering approach for PML (WSC-PML) that bridges clustering and multi-label learning through membership matrix decomposition. Our key innovation decomposes the clustering membership matrix $\mathbf{A}$ into two components: $\mathbf{A} = \mathbf{\Pi} \odot \mathbf{F}$, where $\mathbf{\Pi}$ maintains clustering constraints while $\mathbf{F}$ preserves multi-label characteristics. This decomposition enables seamless integration of unsupervised clustering with multi-label supervision for effective label noise handling. WSC-PML employs a three-stage process: initial prototype learning from noisy labels, adaptive confidence-based weak supervision construction, and joint optimization via iterative clustering refinement. Extensive experiments on 24 datasets demonstrate that our approach outperforms six state-of-the-art methods across all evaluation metrics.

==> sec/6_discussion.tex <==
\section{Discussion}
Our work presents a method for extracting medical-focused representations that addresses key challenges in adapting general-domain models to the medical domain, specifically semantic overlap (mostly caused by data imbalance), and negation handling. Our approach consistently outperforms both baseline and state-of-the-art models across classical tasks and novel benchmarks, demonstrating robustness and effectiveness. Key insights from our findings include: (1) While using negations as hard negatives alone provided limited benefits, combining them with dynamic soft labels significantly improved performance (\cref{ex:main}); (2) our methods enhanced comprehensive clinical understanding, improving performance in adversarial tasks and alignment benchmarks (\cref{ex:cxralign}, \cref{ex:adverserial}); and (3) the inclusion of normal and duplicate reports contributed positively to training on imbalanced datasets, proving valuable insights for general hospital data where data imbalances are common (\cref{ex:normalthinning}).

A potential area for refinement lies in refining the RadGraph~\cite{radgraph}-based graph representation by focusing on structured elements such as \textit{location}, \textit{severity/size}, and \textit{entity}, which could yield more precise clinical representations. Additionally, refining the text encoders~\cite{llm2vec, llm2clip}, with a better understanding of compositional context, remains important.

For clinical similarity, we leveraged CheXbert~\cite{chexbert} outputs rather than embeddings, bypassing some limitations associated with embedding-based similarity measures. However, CheXbert does not encompass all clinical entities, and using more comprehensive labels could further enhance model performance. Future improvements might include embeddings that better capture the unique semantics of chest X-rays, thereby deepening the model’s understanding of clinical relationships. Additionally, exploring alternative similarity measures beyond cosine similarity \cite{lai2024carzero} could yield further improvements.

Our method was designed to integrate text, clinical, and graph similarities to capture the complexity of medical image interpretation in global scale. While results show notable improvements, there remains room to refine this approach for even greater impact in clinical applications.

==> sec/7_conclusion.tex <==

\section{Conclusion}
In this work, we addressed two pivotal challenges in medical vision-language processing—data imbalance and negation handling—by introducing a specialized method that bridges the gap between general and medical domains. Our approach employs clinically-enhanced dynamic soft labels to mitigate semantic overlaps, incorporates negation-based hard negatives to improve the model's comprehension of complex clinical semantics, and integrates graph embeddings while leveraging clinical, relational, and textual similarities. This synergy yields substantial improvements over baseline and state-of-the-art models across various benchmarks. The \textit{CXR-Align} benchmark also highlights our model's superior ability to process negations—an often overlooked yet crucial component in medical reporting. Overall, this study paves the way for more effective medical vision-language models that address the unique challenges of clinical environments, advancing the development of reliable AI tools in healthcare.
